DPOD: 6D Pose Object Detector and Refiner

In this paper we present a novel deep learning method for 3D object detection and 6D pose estimation from RGB images. Our method, named DPOD (Dense Pose Object Detector), estimates dense multi-class 2D-3D correspondence maps between an input image and available 3D models. Given the correspondences, a 6DoF pose is computed via PnP and RANSAC. An additional RGB pose refinement of the initial pose estimates is performed using a custom deep learning-based refinement scheme. Our results and comparison to a vast number of related works demonstrate that a large number of correspondences is beneficial for obtaining high-quality 6D poses both before and after refinement. Unlike other methods that mainly use real data for training and do not train on synthetic renderings, we perform evaluation on both synthetic and real training data demonstrating superior results before and after refinement when compared to all recent detectors. While being precise, the presented approach is still real-time capable.

==> contributions.tex <==
\section{Summary - Presumable Results}

In order to make distinctions among different instances of our methods the following naming conversions will be used:

\begin{itemize}
    \item {\bf DOP}: {\em DOP + PnP with RANSAC}
    \item {\bf End-to-end DOP}: {\em DOP + PnP-Net }
    \item {\bf DOP+NNRef}:  {\em DOP + PnP with RANSAC + Our Neural Network Refinement}
    \item {\bf End-to-end DOP+NNRef}: {\em End-to-end DOP+NNRef: DOP + PnP-Net  + Our Neural Network Refinement}
\end{itemize}

Here we consider {\bf DOP:}{\em DOP + PnP with RANSAC} as our basis method. The refinement is coming on top of it and will be neural network based refinement {\em NNRef}.
The refinement on top of PoseCNN detector is called {\em DeepIM}. I list the expected results and benefits from different method instances listed above.

The results will be generated for both real and synthetic images on LineMOD and LINEMOD Occlusions datasets with and without refinement.

{\em \bf LINEMOD dataset:} The methods we compare with on synthetic will be: SSD6D and AAE, and on real-data we will compare to: BB8, YOLO6D, iPose(from Brachmann), PVNet, PoseCNN, DeepIM(PoseCNN + refinement). 

{\em \bf LINEMOD OCCLUSIONS dataset:} The methods we will compare are actually taken from PVNet paper and contain results of Yolo6D, PoseCNN, Oberweger
all working on real data.

\paragraph{Results on LINEMOD dataset} This is the initial method submitted to CVPR, where UV-maps are regressed. I guess the results will either stay the same or be updated. On synthetic we are better than both SSD6D and AAE without refinement. With refinement I would not put original SSD6D results (edge-based refinement), but results of their NN refiner, which shows just the final ADD score (34,1\% on LineMOD) and (27.5\% on LineMOD OCCLUSIONS). We also need to put results of DeepIM (88.6). In summary the results of related works on LINEMOD can be found in the following tables:

\begin{tabular}{ |l|l|l|l|l| }
\hline
\multicolumn{5}{ |c| }{Synthetic Data} \\
\hline
Method & SSD6D & AAE & DOP & E2E DOP \\ \hline
Mean & 9.1 & 28.65 & 49.98 & \\ \hline
\end{tabular}


\begin{table*}[!ht]
\centering
\caption{Comparison of our approaches DOP+NNRef, E2EDOP+NNRef after refinement to the other refined RGB detectors trained on sythetic data on the LINEMOD dataset. The table reports percentages of correctly estimated poses w.r.t. the ADD score.\label{tab:synthref}}
\begin{tabular}{ |l|l|l|l|l|l|l|l|l| }
\hline
\multicolumn{5}{ |c| }{Synthetic Data} & \multicolumn{4}{ |c| }{Synthetic Data + Refinement} \\ \hline
Method & SSD6D & AAE & DOP & E2E DOP & SSD6D  & AAE & DOP + NNRef & E2E DOP + NNRef \\ \hline
Mean & 9.1 & 28.65 & 49.98 & & 34.1 & 64.67 &  &  \\ \hline
\end{tabular}
\end{table*}

\iffalse
\begin{table*}[!ht]
\centering
\caption{Comparison of our approach DOP before refinement on real data to the other RGB detectors trained on real data on the LINEMOD dataset. The table reports percentages of correctly estimated poses w.r.t. the ADD score.\label{tab:real}}
\begin{tabular}{ |c|c|c|c|c|c|c| }
\hline
\multicolumn{7}{ |c| }{Real Data} \\ \hline
Method & BB8 & YOLO6D & iPose & PoseCNN & DOP & E2E DOP  \\ \hline
Mean & 43.6 & 55.95 & 56.0 & 62.7 & 77.67 & x &  \hline
\end{tabular}
\end{table*}

\begin{table*}[!ht]
\centering
\caption{Comparison of our approach DOP + NNRef after refinement on real data to the other RGB detectors trained on real data on the LINEMOD dataset. The table reports percentages of correctly estimated poses w.r.t. the ADD score.\label{tab:realref}}
\begin{tabular}{ |c|c|c|c|c|c| }
\hline
\multicolumn{6}{ |c| }{Real Data + Refinement} \\ \hline
Method & BB8  & DeepIM & DOP + DeepIM & DOP + NNRef & E2E DOP + NNRef \\ \hline
Mean & 62.7 & 88.6 & 91.8 &  &  & \hline
\end{tabular}
\end{table*}
\fi

\paragraph{Results on LINEMOD Occlusions dataset} Here we present results on Occlusions dataset. The results can be both put in one plot as in our Fig. 6, or a table if we do not have other results with diferent thresholds.

\begin{table*}[!htb]
\centering
\caption{Comparison of our approach DOP on real data to the other RGB detectors trained on real data on the LINEMOD Occlusions dataset. The table reports percentages of correctly estimated poses w.r.t. the ADD score.\label{tab:realoccl}}
\begin{tabular}{ |c|c|c|c|c|c|c|c| }
\hline
\multicolumn{8}{ |c| }{LINEMOD Occlusions} \\ \hline
Method & YOLO  & Ref-SSD6D & PoseCNN & Oberweger & DeepIM  & DOP + NNRef & E2E DOP + NNRef \\ \hline
Mean & 6.42 & 27.5 & 24.9 & 30.4 & 40.77 &   &   \\ \hline
\end{tabular}
\end{table*}
